Homogenization of the Poisson-Nernst-Planck Equations for Ion Transport in Charged Porous Media

Effective Poisson-Nernst-Planck (PNP) equations are derived for macroscopic ion transport in charged porous media under periodic fluid flow by an asymptotic multi-scale expansion with drift. The microscopic setting is a two-component periodic composite consisting of a dilute electrolyte continuum (described by standard PNP equations) and a continuous dielectric matrix, which is impermeable to the ions and carries a given surface charge. Four new features arise in the upscaled equations: (i) the effective ionic diffusivities and mobilities become tensors, related to the microstructure; (ii) the effective permittivity is also a tensor, depending on the electrolyte/matrix permittivity ratio and the ratio of the Debye screening length to the macroscopic length of the porous medium; (iii) the microscopic fluidic convection is replaced by a diffusion-dispersion correction in the effective diffusion tensor; and (iv) the surface charge per volume appears as a continuous "background charge density", as in classical membrane models. The coefficient tensors in the upscaled PNP equations can be calculated from periodic reference cell problems. For an insulating solid matrix, all gradients are corrected by the same tensor, and the Einstein relation holds at the macroscopic scale, which is not generally the case for a polarizable matrix, unless the permittivity and electric field are suitably defined. In the limit of thin double layers, Poisson's equation is replaced by macroscopic electroneutrality (balancing ionic and surface charges). The general form of the macroscopic PNP equations may also hold for concentrated solution theories, based on the local-density and mean-field approximations. These results have broad applicability to ion transport in porous electrodes, separators, membranes, ion-exchange resins, soils, porous rocks, and biological tissues.

==> darcy.tex <==
We briefly restrict ourselves to the Stokes equations contained in our probelm \reff{MaPr}
\bsplitl{
 -\Delta {\bf u}_r +\nabla p_r = {\bf f}_r
 	&\qquad\textrm{in }\Omega^s\,,
 \\
 {\rm div}\,{\bf u}_r = 0
 	&\qquad\textrm{in }\Omega^s\,,
 \\
{\bf u}_r = {\bf 0}
	&\qquad\textrm{on }\partial \Omega^s\,.
 }{eq:PeStokPr}
We are interested in the limit problem for $(p_r,\ol{\rm v}_r)$ as $r\to 0$. Therefore, we first consider the following auxiliary problem on the 
 periodic cell $Y_2:=Y\setminus Y_1$
 \bsplitl{
-\Delta {\bf w}^k +\nabla_y q^k +{\bf e}_k = {\bf 0}
	&\qquad\textrm{in }Y_2\,,
\\
{\rm div}_y\, {\bf w}^k = 0
	&\qquad\textrm{in }Y_2\,,
\\
{\bf w}^k = 0
	&\qquad\textrm{on }\partial Y_1\cap\partial Y_2\,,
\\
{\bf w}^k,\, q^k
	&\qquad\textrm{are $Y$-periodic with respect to }y_1,\dots,y_N\,,
 }{eq:AuxPePr}
 where ${\bf e}_1,\dots,{\bf e}_N$ are the canonical basis functions 
 in $\mathbb{R}^N$. For example by using the two-scale convegence tool, the following passage to the limit from 
 the Stokes problem in a porous medium to Darcy's law is verified for example in \cite{UH} %ChPS, 
and given here without proof for convenience of the reader.
 
 \begin{thm}\label{thm:DarLaw}
 Let ${\bf v}_r$ be a solution of \reff{eq:PeStokPr} extended by 
 zero to $\Omega\setminus \Omega^r$. For all $r>0$ there exists 
 an extension $p_r$ of the pressure to $\Omega\setminus \Omega^r$ such that 
 $\frac{{\bf v}_r}{r^2}\rightharpoonup {\bf v}_0$ weakly in 
 $L^2(\Omega)$ and $p_r\to p_0$ strongly in $L^2(\Omega)$, where 
 $(p_0,{\bf v}_0)$ is a solution of the problem 
 \bsplitl{
 {\rm v}_0^k = {\rm k}_{kl}\brkts{
 	{\rm f}^l - \partial_{x_l}p_0
 	}
 	&\qquad\textrm{in }\Omega\,,
 \\
 {\rm div}\,{\bf v}_0 = 0
 	&\qquad\textrm{in }\Omega\,,
 \\
 \brkts{{\bf v}_0,\ol{\nu}} = 0
 	&\qquad\textrm{on }\partial \Omega\,,
 }{eq:HoStok}
 and ${\rm v}_0^k$ is the $k$-th component of the vector-valued function 
 ${\bf v}_0$, and $\pmb{\nu}$ is the outward normal to $\partial \Omega$ 
 and the matrix ${\rm k}_{kl}$ is called the Darcy matrix and defined by
 \bsplitl{
 {\rm k}_{kl}:=\frac{1}{\av{Y}}\int_{Y_2}{\rm w}_l^k\,dy\,,
 }{eq:DarMat}
 for solutions ${\rm w}_l^k$ of \reff{eq:AuxPePr} with index $l$ denoting the 
 $l$-th component of the vector ${\bf w}^k$.
\end{thm}


==> pmPNP.tex <==
\subsection{Microscopic model}\label{sec:MiEq}
Our derivation begins with a periodic representation of the microstructure and uses a formal two-scale convergence method to derive effective equations valid at scales much larger than the geometrical period, as sketched in Figure \ref{fig:perReCe}. Schmuck~\cite{Schmuck2010} recently applied this approach to derive effective PNP equations for ion transport with convection in uncharged porous media. The extension to fluid flow for the full nonlinear PNP equations in a charged microstructure is still lacking a consistent 
derivation, as pointed out in~\cite{Schmuck2011}. Indeed, the classical theory of electrokinetic phenomena in porous media (e.g. streaming potential, electro-osmotic flow, diffusio-osmosis) assumes linear response to small perturbations~\cite{hunter_book}, but it has only recently been understood that many nonlinear electrokinetic phenomena, such as second-kind electro-osmotic flows~\cite{leinweber2004,tallarek2005}, induced-charge electro-osmotic flows~\cite{iceo2010},  
deionization shocks~\cite{Mani2010,Mani2009}, and surface-driven over-limiting current~\cite{dydek2011}, can arise due to the coupling between ion transport and surface charge in microstructures. Hence, we neglect flow, but we allow for a fixed surface charge density on the solid or molecular matrix. In the following sections, we emphasize physical implications and provide some illustrative examples.

Suppose that the heterogeneities, 
i.e. the size of the pores defined by a reference cell $Y$, as for example in Figure \ref{fig:Cors1} left (in 2D), are very small with respect to the size of the porous medium denoted by $\Omega\subset\mathbb{R}^d$, $1\leq d\leq 3$, and that they are evenly distributed. This is a realistic assumption for a large class of applications. 
From a mathematical point of view, one can model this distribution by supposing that it is a periodic one. In fact, to reduce the approximation error, one can first compute the averaged pore structure of a suitable periodic replacement by a so-called Y-Algorithm, see \cite{Schmuck2010}. The periodicity can be represented by a small parameter $r$ and hence the porous subset $\Omega^p$ 
of $\Omega$ is then denoted by $\Omega^p_r$ and correspondingly the solid subset $\Omega^s$ by $\Omega^s_r:= \Omega\setminus \Omega^p_r$. For the moment, we assume that the solid-electrolyte interface 
$I_r:=\partial \Omega^p_r\cap \partial \Omega^s_r$ is smooth. Further, we suppose that we are given a reference period $Y$, in which the reference heterogeneities are defined, see Figure \ref{fig:Cors1} left (in 2D) respectively Figure \ref{fig:Cors1} right (in 3D). The pores in $\Omega$ are periodic of period $r Y$ and their size is of order $r$. The concentration densities $c^\pm$ have to be solved only in the domain of the liquid phase which is the perforated domain $\Omega^p_r=\Omega\setminus \Omega^s_r$. Then, for the scaling parameter $r>0$, 
the positive ion density $c^+_r$, negative ion density $c^-_r$, 
and the electrostatic potential $\phi_r$ are governed by the equations 
\bsplitl{
{\textrm{\bf{(micro PNP)}}}\qquad
\begin{cases}
\partial_t c^+_r 
	= {\rm div}\brkts{\nabla c^+_r + c^+_r\nabla\phi_r}
	&\qquad\textrm{in }\Omega_r^p\,,
\\
\partial_t c^-_r 
	= {\rm div}\brkts{\nabla c^-_r - c^-_r\nabla\phi_r}
	&\qquad\textrm{in }\Omega_r^p\,,
\\
-{\rm div}\brkts{\varepsilon(x/r)\nabla\phi_r}
	= c^+_r-c^-_r
	&\qquad\textrm{in }\Omega:=\Omega^p_r\cup\Omega^s_r\,,
\end{cases}
}{perPNP}
where $\varepsilon(x):=\epsilon^2\chi_{\Omega^p_r}(x)
+\alpha\chi_{\Omega^s_r}(x)$, $\epsilon:=\frac{\lambda_D}{\ell}$ the dimensionless Debye length, and 
$\alpha:=\frac{\varepsilon_s}{\varepsilon_p}$ the dimensionless electric 
permittivity of the solid material $\varepsilon_s$ scaled to that of the pore phase $\varepsilon_p$. The system (\ref{perPNP}) is completed by the boundary conditions
\bsplitl{
\nabla_n c^+_r +
c^+_r\nabla_n\phi_r
	= 0
	&\qquad\textrm{on }I_r:=\partial \Omega^p_r\cap \partial \Omega^s_r\,,
\\
\nabla_n c^-_r -c^-_r\nabla_n\phi_r
	= 0
	&\qquad\textrm{on }I_r\,,
\\
-\varepsilon(x/r)\nabla_n\phi_r
%\ebrkts{\brcs{\varepsilon(x/r)\nabla_n\phi_r}\Bigl|_{\partial\Omega^p_r}
%		-\brcs{\varepsilon(x/r)\nabla_n\phi_r}\Bigl|_{\partial\Omega^s_r}}
	=r\sigma_{\rm s}(x/r)
	&\qquad\textrm{on }I_r\,,
}{pBC}
where $\sigma_{\rm s}(x/r)$ is a periodic surface charge density. Since we describe the solid-electrolyte composite 
by macroscopic respectively continuous variables, we do not model the surface charge by a jump boundary 
condition. In Figure \ref{fig:perReCe}, we illustrate the periodic 
formulation (\ref{perPNP})--(\ref{pBC}), which allows to introduce a periodic reference cell $Y:=Y^p\cup Y^s$ capturing the pore geometry. 

\begin{figure}
	\centering
	\includegraphics[height=8cm,width=14cm]{pics/periodicRefCellExpl1.png}%periodicRefCellExpl.png}
	\caption{{\bf Left, macro scale:} Domain $\Omega:=\Omega^p_r\cup\Omega^s_r$ with the solid-liquid interface 
	$I_r:=\partial\Omega^p_r\cap\partial\Omega^s_r$. {\bf Right, micro scale:} Reference cell 
	$Y:=Y^p\cup Y^s:=[0,\ell_1]\times[0,\ell_2]$ with solid-liquid interface $S:=Y^p\cap Y^s=I_r\cap Y$. The micro scale is obtained by rescaling the macro scale 
	with the parameter $r$ which measures the characteristic size of the heterogeneities. The upscaling or averaging 
	process then consists in passing to the limit $r\to 0$, i.e. the electrolyte and the solid phase are homogeneously 
	mixed under keeping the corresponding volume fractions constant.}
	\label{fig:perReCe}
\end{figure}

\medskip


\subsection{ Macroscopic approximation }\label{sec:MaEq}
A formal application of the two-scale convergence allows to derive the following upscaled 
equations describing electrolytes in porous media for fixed surface charge. The basic idea 
is an asymptotic approximation of the form
\bsplitl{
c^\pm_r(t,x) 
	& \approx \brkts{1+r\delta_{c^\pm}^l(x/r)\partial_{x_l}+{\cg O}(r^2)} c_0^\pm(t,x)\,,
\\
\phi_r(t,x) 
	& \approx \brkts{1+r\delta_{\phi}^l(x/r)\partial_{x_l}+{\cg O}(r^2)} \phi_0(t,x)\,,
}{AsAp}
where Einstein's summation convention is applied over repeated indices and the microscopic variable 
$y=x/r\in Y$ is used. We point out that the series in \reff{AsAp} are not necessarily convergent. 
By $Y$ we denote the reference cell which captures the geometric and interfacial information of the microstructure.  

It is important to stress that we use dimensionless length and time variables (\ref{RV}) scaled to the characteristic length and time scales for diffusion across a reference cell at the scale of individual pores. This is convenient for homogenization and allows us to vary the Debye length relative to the mean pore size (below). In applications of the macroscopic PNP equations obtained by homogenization, however, it is better to rescale length and time according to the scales of bulk diffusion across $r^{-1}\gg 1$ reference cells over a length $L=\ell/r$ in terms of the following macroscopic dimensionless variables:
\begin{equation}
\bar{\epsilon} = \frac{\lambda_D}{L} = r \epsilon, \ \  \ 
\bar{x} = \frac{x}{L} = r \tilde{x}, \ \ \ 
\bar{\nabla} = L \nabla = r^{-1} \tilde{\nabla}, \ \  \ 
\bar{t} = \frac{t D}{L^2} = r^2 \tilde{t} \label{macro}
\end{equation}
This rescaling will be useful below when we consider the limit of thick double layers compared to the pore size ($\epsilon \ll 1$), which could be thin ($\bar{\epsilon} \ll 1$) or thick  ($\bar{\epsilon} \gg 1$)  at the macroscopic geometrical scale.

Without further 
details, we directly state here the main result which extends the derivations in \cite{Schmuck2010,Schmuck2012} 
to the case of charged porous materials. We further generalize \cite{Schmuck2010} 
under local thermodynamic equilibrium as achieved in \cite{Schmuck2011,Schmuck2012}. The article \cite{Schmuck2012} additionally qualitatively characterizes the effective porous media approximation of the PNP equations by quantitative 
error estimates.

The following definition guarantees the well-posedness of the effective porous media approximation 
subsequently presented. It can also be justified on both physical and mathematical grounds by the assumed separation of the macroscopic and microscopic length scales, analogous to the quasi-equilibrium  approximation for thin double layers.

\begin{defn}\label{def:LoEq} \emph{(Local thermodynamic equilibrium in dilute solutions)} We say that for dilute solutions the reference cells $Y$ 
are in local thermodynamic equilibrium if and only if,
\bsplitl{
\mu_0^i := {\rm log}\,c^i(t,x) +z_i\phi(t,x)
	= {\rm const.}
	\qquad\textrm{in }x/s=y\in Y\,,
}{LoEqCo}
where $\mu_0^i$ denotes a constant value of the chemical potential of positive ($i=+$) 
and negative ($i=-$) ion densities and $z_\pm := \pm 1$. 
The locally constant potential $\mu_0^i$ can assume different values in different reference cells.
\end{defn}

\begin{rem}\label{rem:LoEq}
We emphasize that the equilibrium condition \reff{LoEqCo} specifically accounts for dilute 
solutions. For the more general concentrated solution theory, a corresponding equilibrium 
is defined in \reff{ChPoEx}.
\end{rem}

Under local thermodynamic equilibrium, the effective positive ion density $c^+$, effective concentration of negative ions $c^-$, and the effective electric 
potential $\phi$ are determined by
\bsplitl{
\textrm{\bf{(macro PNP)}}
\qquad
\begin{cases}
p\partial_tc^+
	= {\rm div}\brkts{\hat{\rm D}\nabla c^+ 
		+c^+\hat{\rm M}\nabla\phi}\,,
	&\qquad\textrm{in }\Omega\,,
\\
p\partial_t c^-
	={\rm div}\brkts{
              \hat{\rm D}\nabla c^- 
		-c^-\hat{\rm M} \nabla\phi
	}\,,
	&\qquad\textrm{in }\Omega\,,
\\
-{\rm div}\brkts{\hat{\varepsilon}(\epsilon,\alpha)\nabla\phi} 
	= p\brkts{c^+-c^-} 
	+ \rho_{\rm s}\,,
	&\qquad\textrm{in }\Omega\,,
\end{cases}
}{pmPNP}
where $\rho_{\rm s}:=\frac{1}{\av{Y}}\int_{\partial Y_1 \cap \partial Y_2}\sigma_{\rm s}\,do(y)
$ is the total surface charge per volume (which plays the role of the ``background charge" in classical membrane and semiconductor models), 
$\alpha :=\frac{\varepsilon_s}{\varepsilon_p}$ is the permittivity ratio, 
$\epsilon := \sqrt{\frac{\varepsilon_pkT}{2e^2C_0}}/\ell$  is the dimensionless Debye length (measuring the thickness of the double layers), and the different 
tensors $\hat{\rm D}:=\brcs{{\rm d}_{kl}}_{1\leq k,l\leq d}$, $\hat{\rm M}:=\brcs{{\rm m}_{kl}}_{1\leq k,l\leq d}$, 
and $\hat{\varepsilon}(\epsilon,\alpha):=\brcs{\varepsilon_{kl}(\epsilon,\alpha)}_{1\leq k,l\leq d} $ are defined by  
\bsplitl{
& {\rm d}_{kl}
	= \frac{1}{\av{Y}}\int_{Y^s}
	\brcs{
		\delta_{kl} - \delta_{kj}\partial_{y_j}\xi^{ii_l}(y)
	}\,dy\qquad\textrm{for }i=1,2\,,
\\&
{\rm m}_{kl}
	= \frac{1}{\av{Y}}\int_{Y^s}
	\brcs{
		\delta_{kl} - \delta_{kj}\partial_{y_j}\xi^{33_l}(y)
	}\,dy\qquad\textrm{for }i=1,2\,,
\\&
\varepsilon_{kl}(\epsilon,\alpha)
	= \frac{\lambda^2}{\av{Y}}\int_{Y^s}
	\brcs{
		\delta_{kl} - \delta_{kj}\partial_{y_j}\xi^{33_l}(y)
	}\,dy
	+\frac{\alpha}{\av{Y}}\int_{Y\setminus Y^s}
	\brcs{
		\delta_{kl} - \delta_{kj}\partial_{y_j}\xi^{33_l}(y)
	}\,dy\,.
}{s33}
The corrector functions 
$\xi^{ii_r}$ solve for $i=1,2,3$ and $1\leq r\leq d$ the reference cell problems
\bsplitl{
\begin{cases}
\quad- \Delta_y (\xi^{ii_r}-y_r)
	= -\Delta_y(\xi^{33_r}-y_r)
	& \qquad\textrm{in }Y^s\,,
\\
\qquad\qquad\brkts{-\nabla_y(\xi^{ii_r}-y_r)
	+\nabla_y(\xi^{33_r}-y_r)}\cdot {\rm n}_I
	=0
	&\qquad\textrm{on }I:=\partial Y^s\,,
\\
\qquad\qquad {\xi}^{ii_r}\textrm{ is $Y^s$-periodic and ${\cg M}_{Y^s}({\xi}^{ii_r})=0$}\,,
	&
\\
\quad- {\rm div}_y\brkts{\hat{\varepsilon}(y)\nabla_y(\xi^{33_r}-y_r)}
	= 0
	& \qquad\textrm{in }Y\,,
\\
\qquad\qquad\xi^{33_r}\textrm{ is $Y$-periodic and 
${\cg M}(\xi^{33_r})=0$}\,.
	&
\end{cases}
}{ChCoEq}
As a consequence of (\ref{ChCoEq}), it holds $\xi^{11_r}=\xi^{22_r}$.
The quantity $\partial Y^s$ denotes the boundary of the solid phase in the 
reference cell $Y=Y^s\cup Y^p$ and is part of the interface $I$ on the domain $\Omega$, see for 
example Figure \ref{fig:Cors1} left. The subset $Y^s$ denotes the solid phase (black in Figure \ref{fig:perReCe}) and $Y^p$ the electrolyte phase (blue in Figure \ref{fig:perReCe}). Furthermore, the effective tensors
(\ref{s33})$_1$--(\ref{s33})$_2$ contain relevant macroscopic corrections defined by 
the microscopic pore structure. We remark that the corrector 
${\varepsilon}_{kl}(\epsilon,\alpha)$ for the Poisson equation (\ref{pmPNP})$_3$ is equal to $\hat{\rm D}_{kl}$ defined in (\ref{s33})$_1$, if and only if we assume that the 
electric field only exists in the electrolyte phase. Such an assumption is equivalent to the 
limit $\alpha\to 0$, see Section \reff{sec:InPoMa}. The correction tensor $\hat{\rm D}_{kl}$ can only be motivated analytically in the case of straight channels, see Section \ref{sec:StCh} and \cite{Auriault1993}. Already for perturbed straight channels, a numerical approach is required to solve the reference cell problem (\ref{ChCoEq}). We refer to Section \ref{sec:PeStCh} and \cite{Auriault1997} 
for further details.

Finally, we motivate that the assumption of local thermodynamic equilibrium \reff{LoEqCo} guarantees 
solvability of the reference cell problem \reff{ChCoEq}. As demonstrated in \cite{Schmuck2011}, 
\reff{ChCoEq}$_1$ is obtained as the ${\cg O}(r^{-1})$-order problem for an asymptotic 
expansion \reff{AsAp}. That means, for arbitrary smooth test functions $\Psi^i$, $i=1,2$, we first obtain 
\bsplitl{
& \sum_{k,l=1}^N\biggl\{
	\brkts{
	\brkts{
		\delta_{kl}\partial_{y_l}\xi^{ii_r},\partial_{y_k}\Psi^{i}
	}_{Y^s}
	-\brkts{
		\delta_{kr},\partial_{y_k}\Psi^i
	}_{Y^s}
	}\partial_{x_r}c^i
\\&\qquad
	+\brkts{
	\brkts{
		c^i\delta_{kl}\partial_{y_l}\xi^{33_r},\partial_{y_k}\Psi^i
	}_{Y^s}
	- \brkts{
		c^i\delta_{kr},\partial_{y_k}\Psi^1
	}_{Y^s}
	}z_i\partial_{x_r}\phi
	\biggr\}
	=0
	\quad\textrm{for }i=1,2\,,
}{Or-1}
where $c^1=c^+$, $c^2=c^-$, $z_1=+1$, and $z_2 = -1$. The notation $(u,v)_D:=\int_D uv\,dx$ denotes 
the scalar product in $L^2(D)$-sense with $D=Y^s$. In classical homogenization theory, one can immediately 
cancel out macroscopic quantities like $\partial_{x_r} c^i$. This is here not possible due to the additional gradient of 
the electric potential $\partial_{x_r}\phi$. Since we do not exactly know when $\partial_{x_r}c^i(x,t)$ becomes zero, we cannot immediately apply Lax-Milgram's theorem or the Fredholm alternative in order to 
guarantee solvability of \reff{Or-1}. But under the local equilibrium assumption \reff{LoEqCo}, we are 
able to remove the macroscopic quantities $\partial_{x_r}c^i$ and $z_i\partial_{x_r}\phi$ such 
that we end up with equation \reff{ChCoEq}$_1$. Solvability of \reff{ChCoEq}$_1$ then 
immediately follows via Lax-Milgram's theorem.

\subsection{Einstein relations}\label{sec:EiSt}
The upscaled PNP equations indicate that Einstein's relation between diffusion $D$ and mobility $M$
coefficient, i.e., $M=\frac{D}{kT}$, does not hold with respect to the porous media correction tensors $\hat{\rm D}$ 
and $\hat{\rm M}$.
At first, this seems to be physically inconsistent, since we seem to loose the gradient flow structure 
\reff{NP} and a Boltzmann distribution for ion densities in equilibrium.

However, we point out that the tensors $\hat{\rm D}$ and $\hat{\rm M}$ are corrections to 
$\nabla c^\pm$ and $\nabla\phi$, respectively, and not to diffusion and mobility coefficients. This 
important fact then motivates to define the mean field approximations 
\bsplitl{
\ol{\nabla c^\pm}	
	& :=\hat{\rm D}\nabla c^\pm\,,
\\
\ol{\nabla\phi}
	& :=\hat{\rm M}\nabla\phi\,.
}{MfAp}
It is immediately clear that the Einstein relation holds for the quantities \reff{MfAp}, i.e., 
$D_\pm\ol{\nabla c^\pm}+kTz_\pm M_\pm \ol{\nabla\phi} = kT M_\pm\ol{\nabla\mu}_\pm$ in dimensional variables. 
Moreover, via \reff{MfAp} we can define a mean field gradient of the 
chemical potential by
\bsplitl{
\ol{\nabla\mu}_\pm
	& := 
	\frac{\delta\mu}{\delta c^i}\ol{\nabla c^i}	
	+ z_i\frac{\delta\mu}{\delta \phi}\ol{\nabla\phi}
	= \frac{1}{kT} \frac{\delta\mu}{\delta c^i}\hat{\rm D}\nabla c^i	
	+ \frac{\delta\mu}{\delta \phi}\hat{\rm M}\nabla\phi\,,
}{MfChPo}
such that gradient flow \reff{NP} becomes,
\bsplitl{
\partial_tc^\pm
	= - {\rm div}\brkts{- c^\pm M\ol{\nabla\mu_\pm}}\,,
}{GrFl}
where $M=M_\pm =\frac{D_\pm}{kT}$. 
We further remark that the mean field approximation \reff{MfChPo} is only defined for 
the gradient of the chemical potential. This fact is a direct consequence of the 
Ansatz \reff{AsAp}. As a consequence, the chemical potential $\mu_\pm$ remains 
unchanged and hence Boltzmann's distribution for the ion densities still 
holds in thermodynamic equilibrium.

\subsection{Material tensor and Onsager relations}\label{sec:MaTe}

In \cite{Schmuck2010}, it is shown that the definitions (\ref{s33})$_1$--(\ref{s33})$_3$ allow to introduce a so-called effective material tensor 
\bsplitl{
\hat{\rm S}_{i_kj_l}({\bf Q}) := 
\ebrkts{
\begin{array}{ccc}
\hat{\rm D}_{kl} 
& 
0 
& Q^2\hat{\rm M}_{kl}  
\\
0 
& \hat{\rm D}_{kl}  
& -Q^1\hat{\rm M}_{kl}  
\\
0 
& 0 
& \hat{\varepsilon}_{kl}(\epsilon,\alpha)  
\end{array}
}\,,
}{HoTeEx}
which allows to write \reff{pmPNP} for the field vector ${\bf Q}:=[c^+,c^-,\phi]'$ and the 
right-hand side ${\bf I}({\bf Q}):=[0,0,Q^1-Q^2]'$ by
\bsplitl{
\pmb{\partial}_{\bf t} {\bf Q}
	+ {\bf div}\brkts{\hat{\rm S}({\bf Q})\pmb{\nabla}{\bf Q}}
	= {\bf I}({\bf Q})\,,
}{CoNo}
where $\pmb{\partial}_{\bf t}$ is the operator
\bsplitl{
\pmb{\partial}_{\bf t}
	:= \begin{bmatrix}
	\partial_t & 0 & 0 \\
	0 & \partial_t & 0 \\
	0 & 0 & 0 
	\end{bmatrix}\,,
}{TiDeOp}
and also $\pmb{\nabla}$ and $\pmb{\rm div}$ are correspondingly defined.

\begin{rem}\label{rem:Eps} Let us point out the special case where the electric field 
only exists in the electrolyte phase. In such situations, the tensor $\hat{\varepsilon}_{kl}(\epsilon,\alpha)$ in (\ref{HoTeEx}) can be replaced by $\epsilon^2\hat{\rm D}_{kl}$, see Section \reff{sec:InPoMa}.
\end{rem}

The material tensor (\ref{HoTeEx}) provides a ``nonlinear equivalent'' to the Onsager relations for situations apart from thermodynamic equilibrium. It is completely determined by the elementary cell $Y$ as 
for example given in Figure \ref{fig:Cors1} left (in 2D) and right (in 3D), respectively the equations (\ref{s33})-(\ref{ChCoEq}). Such 
a reference cell represents the characteristic geometry of the porous material under consideration. 
The material tensor $\hat{\rm S}$ relates the gradients of concentrations and electric potential 
to their corresponding fluxes ${\bf J}:=[{\rm J}_{c^+},{\rm J}_{c^-},{\rm J}_{\phi}]'$, i.e.
\bsplitl{
{\bf J} = \hat{\rm S}({\bf Q})\nabla{\bf Q}\,.
}{FlRe} 
The classical Onsager reciprocal relations only hold true for a linearized 
material tensor \reff{HoTeEx}. In fact, Allaire et al.~\cite{allaire2010} rigorously achieve the Onsager relations,  
first verified in Looker and Carnie~\cite{looker2006}, for a linearized and time-independent version of ionic transport 
in contrast to the full nonlinear problem considered here. 

Next to the physical information gained by the transport parameters 
in the tensor (\ref{HoTeEx}), the effective equations (\ref{pmPNP}) also prevent high-dimensional 
and hence computationally expensive problems. Such computationally demanding 
situations generally result by solving (\ref{PNP}) over the real microstructure. In fact, the mesh for 
such computations is required to be smaller than the characteristic 
length scale $r$ of the heterogeneities. 

Let us mention that it is not possible to derive (\ref{pmPNP}) by volume averaging 
or the representative volume mehtod (RVM), since the system (\ref{PNP}) is nonlinear. Moreover, 
it is not clear what is the right size of the test volumes with respect to which the 
gradients and their corresponding fluxes are averaged. Also a possible dependence on a source term and boundary 
conditions, see (\ref{pBC})$_3$, cannot be captured by such approaches. These reasons strongly motivate the 
effective equations (\ref{pmPNP}) derived here by homogenization techniques.

\subsection{Reformulation of \reff{pmPNP} for salt and charge variables}\label{sec:ReFo}

Finally, we reformulate (\ref{pmPNP}) for the physical quantities charge $\rho$ and salt $c$, i.e.
\bsplitl{
p\partial_t\rho
	= {\rm div}\brkts{\hat{\rm D}\nabla \rho 
		+c\hat{\rm M}\nabla\phi}\,,
	&\qquad\textrm{in }\Omega\,,
\\
p\partial_t c
	={\rm div}\brkts{
              \hat{\rm D}\nabla c 
		+\rho\hat{\rm M} \nabla\phi
	}\,,
	&\qquad\textrm{in }\Omega\,,
\\
-{\rm div}\brkts{\hat{\varepsilon}(\epsilon,\alpha)\nabla\phi} 
	= p\rho
	+ \rho_{\rm s}\,,
	&\qquad\textrm{in }\Omega\,,
}{pmPNPSaCh}

where we call $\hat{\kappa}:=\rho\hat{\rm M}$ the macroscopic conductivity. $\hat{\rm D}$ and 
$\hat{\rm M}$ are microscopic correction tensors which contain the information 
about the pore geometry. 

There is a growing body of recent theoretical and experimental work on ion transport in charged nanopores. If the 
Debye length is smaller than the pore radius, then continuum models can agree very well with 
experimental data \cite{Ramirez2003}. The mathematical description of ion transport in various recent models \cite{Ramirez2007,Szymczyk2010,Mani2009,Mani2010,dydek2011} has a similar form as our porous-media PNP system (\ref{pmPNPSaCh}),  but without making any connection between the microstructure and the macroscopic coefficients in the equations.  In particular, the hydrodynamic factors $K_{i,d}$ and $K_{i,c}$ used in \cite{Szymczyk2010} 
are not systematically derived and not defined by the pore geometry
as $\hat{\rm D}$ and $\hat{\rm M}$ in \reff{s33} and (\ref{ChCoEq}). Moreover, the cross-sectional area averaging developed by \cite{Ramirez2007} and \cite{Mani2009} was only applied to straight, symmetric channels.

\subsection{Insulating porous matrix}\label{sec:InPoMa}
As indicated in Remark \ref{rem:Eps}, the porous media correction $\hat{\varepsilon}(\epsilon,\alpha)$ 
for the Poisson equation can be reduced to $\hat{\rm D}$ in the case of an insulating 
porous material. As a consequence, also $\hat{\rm M}$ reduces to $\hat{\rm D}$ and hence the material tensor \reff{HoTeEx} simplifies to
\bsplitl{
\hat{\rm S}_{i_kj_l}({\bf Q}) := 
\ebrkts{
\begin{array}{ccc}
\hat{\rm D}_{kl} 
& 
0 
& Q^2\hat{\rm D}_{kl}  
\\
0 
& \hat{\rm D}_{kl}  
& -Q^1\hat{\rm D}_{kl}  
\\
0 
& 0 
& \epsilon\hat{\rm D}_{kl}  
\end{array}
}\,.
}{HoTeEx2}
Let us introduce the following coordinate tranformation
\bsplitl{
\tilde{x} := \hat{\rm D}^{-1/2}x\,,
}{CoTr}
where components of $\tilde{x}$ admitting ``$\infty$'' are subsequently to be treated as parameters.
This coordinate transformation can also be interpreted from a more experimental view point, since there is a 
close relation to tortuosity and diffusivity, see Section \ref{sec:Tor} for details.
With \reff{CoTr} the gradient $\nabla_x$ and the divergence operator ${\rm div}_x$ change with respect to 
the new coordinates to
\bsplitl{
\nabla_x = \hat{\rm D}^{-1/2}\nabla_{\tilde{x}}\,,
	\quad\textrm{and}\quad
	{\rm div}_x  
	= (\nabla_x)'
	= {\rm div}_{\tilde{x}} \hat{\rm D}^{-1/2}\,.
}{TrOp}
Via \reff{TrOp}, the tensor \reff{HoTeEx2} can be written in this new 
coordinates $\tilde{x}$ by
\bsplitl{
\hat{\rm M}_{i_kj_l}(\tilde{\bf Q}) := 
\ebrkts{
\begin{array}{ccc}
1
& 
0 
& \tilde{Q}^2 
\\
0 
& 1 
& -\tilde{Q}^1
\\
0 
& 0 
& 1  
\end{array}
}\,,
}{HoTeEx3}
where $\tilde{Q}(t,\hat{\rm D}^{1/2}\tilde{x})=Q(t,x)$.
Hence, the material tensor \reff{HoTeEx2} takes the same form in the new coordinates 
$\tilde{x}$ as the classical PNP eqations for homogeneous media in the case of an 
insulating porous matrix. Moreover, the porous media equation \reff{CoNo} reads in the new 
coordinates as 
\bsplitl{
\pmb{\partial}_{\bf t} \tilde{\bf Q}
	+ {\bf div}_{\tilde{x}}\brkts{\hat{\rm M}(\tilde{\bf Q})\pmb{\nabla}_{\tilde{x}}\tilde{\bf Q}}
	= {\bf I}(\tilde{\bf Q})\,.
}{TrCoNo}
Let us remark that the transformation \reff{CoTr} accounts for a finite separation of scales and can be 
generalized to the case of a continuum of scales by the idea of metric-based upscaling 
introduce in \cite{Owhadi2007}.

\subsection{Concentrated solution theory}\label{sec:CoSo}  
%We assume that the porous material is an insulating matrix as analyzed in the previous Section 
%\reff{sec:InPoMa}. 
We briefly consider arbitrary chemical potentials (\ref{ChPoEx}) satisfying the local density approximation, i.e. depending only on local concentrations and the potential. In that case, the gradient flow \reff{NP} 
can be accordingly obtained for species $c^i$ and electric potential $\phi$. To this end, 
we first compute the gradient of the chemical potential \reff{ChPo}, i.e. 
\bsplitl{
\nabla\mu(c^i,\phi)
	= \frac{\delta\mu}{\delta c^i}\nabla c^i	
	+ \frac{\delta\mu}{\delta \phi}\nabla\phi\,.
}{1VaChPo2}
If the first variations $\frac{\delta\mu}{\delta c^i}$ and $\frac{\delta\mu}{\delta \phi}$ are linear, then the form of the upscaled equations can be verified as in Section \ref{sec:FoDeTwSc}. For nonlinear $\frac{\delta\mu}{\delta c^i}$ 
and $\frac{\delta\mu}{\delta \phi}$, the multiple-scale method \reff{AsAp} allows us to at least formally obtain the structure of the homogenized equations. In light of the explanations after \reff{1VaChPo2}, we expect that the general porous media formulation for LDA models takes the same basic form
\bsplitl{
p\partial_t c_i
	:= -{\rm div}\brkts{-M_{i}\ol{\nabla\mu}(c_j,\phi)}
}{pmMoFl}
where $\ol{\nabla\mu}$ is defined as in \reff{MfChPo}
and we allow for a multicomponent electrolyte, as well as (formally) for nonlinearities in the mobilities. 

\section{Formal derivation of the upscaled equations by the two-scale convergence method}\label{sec:FoDeTwSc}

\begin{figure}[htbp]
\begin{center}
\setlength{\unitlength}{0.8cm}
\begin{picture}(14,6)(0,0)					% \begin{picture}(width,height)(x-offset,y-offset), 
									% 				offset = lower left corner
\thicklines
\multiput(0.0,0.0)(0.8,0.0){6}{\framebox(0.8,0.8)[s]{\put(0.4,0.0){\circle*{0.6}}}}
\multiput(0.0,0.8)(0.8,0.0){6}{\framebox(0.8,0.8)[s]{\put(0.4,0){\circle*{0.6}}}}
\put(-0.5,1.6){\line(1,0){0.5}}
\multiput(0.0,1.6)(0.8,0.0){6}{\framebox(0.8,0.8)[s]{\put(0.4,0){\circle*{0.6}}}}
\put(-0.5,2.4){\line(1,0){0.5}}
\put(-0.25,1.6){\vector(0,1){0.8}}
\put(-0.25,2.4){\vector(0,-1){0.8}}
\put(-0.6,1.9){$r$}
\multiput(0.0,2.4)(0.8,0.0){6}{\framebox(0.8,0.8)[s]{\put(0.4,0){\circle*{0.6}}}}
\multiput(0.0,3.2)(0.8,0.0){6}{\framebox(0.8,0.8)[s]{\put(0.4,0){\circle*{0.6}}}}
\put(0,5.0){Strongly heterogeneous}
\put(0,4.5){material, i.e. $0<r\ll 1$}
\put(6.4,2.25){($r\to 0$)}
\put(6.0,2.0){\vector(2,0){2.0}}
\put(9.5,0.0){\fcolorbox{black}{grau}{\makebox(4.8,4.0)[]{}}} %
\put(9.3, 4.5){Homogenous approximation}
\end{picture}
\caption{{\bf Left:} A composite material whose characteristic heterogeneity has the lenth $r$. 
{\bf Middle:} Passing to the limit $r\to 0$ under constant volume fraction between circle and square. 
{\bf Right:} The limit problem is obtained with the theory of homogenization.} 
\label{fig:3.1}
\end{center}
\end{figure}

In Figure \ref{fig:3.1} we recall the basic idea behind the homogenization method. For the upscaling process, we first write the system (\ref{perPNP}) 
in the distributional sense. Therefore, we multiply equations 
(\ref{perPNP})$_1$ and (\ref{perPNP})$_2$ by 
a smooth function $\varphi\in C^\infty(\Omega^p_r)$ and 
the Poisson equation (\ref{perPNP})$_3$ with 
$\varphi\in C^\infty(\Omega)$. After integration over $\Omega^p_r$ and $\Omega$, we end up with the formulation
\bsplitl{
\brkts{\partial_t c^+_r,\varphi}_{\Omega^p_r}
	& = \brkts{\nabla c^+_r+c_r\nabla\phi_r,\nabla\varphi}_{\Omega^p_r}
	+\int_{I_r}\brcs{\nabla \rho_r
		+ c_r\nabla\phi_r}\varphi {\bf n}\,do(x)\,,
\\
\brkts{\partial_t c^-_r,\varphi}_{\Omega^p_r}
	& = \brkts{\nabla c^-_r+c^+_r\nabla\phi_r,\nabla\varphi}_{\Omega^p_r}
	+\int_{I_r}\brcs{\nabla c^-_r
		+c^+_r\nabla\phi_r}\varphi {\bf n}\,do(x)\,,
\\
-\brkts{\varepsilon(x/r)\nabla\phi_r,\nabla\varphi}_\Omega
	& = \brkts{c^+_r-c^-_r,\varphi}_\Omega
	-\int_{I_r}
	%\ebrkts{
	%	\brcs{
		\hat{\varepsilon}(x/r)\nabla\phi_r %}\Bigl|_{\partial\Omega^p_r}
	%	-\brcs{\varepsilon(x/r)\nabla\phi_r}\Bigl|_{\partial\Omega^s_r}}
		\varphi{\bf n}\,do(x)\,.
}{DiFo}
With the boundary conditions (\ref{pBC}), the system (\ref{DiFo}) reduces 
to
\bsplitl{
\brkts{\partial_t c^+_r,\varphi}_{\Omega^p_r}
	& = \brkts{\nabla c^+_r+c^-_r\nabla\phi_r,\nabla\varphi}_{\Omega^p_r}\,,
%	+\int_{\partial\Omega_r^1}\brcs{\nabla\rho_r
%		+c_r\nabla\phi_r}\varphi {\bf n}\,do(x)\,,
\\
\brkts{\partial_t c^-_r,\varphi}_{\Omega^p_r}
	& = \brkts{\nabla c^-_r+c^+_r\nabla\phi_r,\nabla\varphi}_{\Omega^p_r}\,,
%	+\int_{\partial\Omega_r^1}\brcs{\nabla c_r
%		+\rho_r\nabla\phi_r}\varphi {\bf n}\,do(x)\,,
\\
-\brkts{\varepsilon(x/r)\nabla\phi_r,\nabla\varphi}_\Omega
	& = \brkts{c^+_r-c^-_r,\varphi}_\Omega
	+r\int_{I_r}\sigma_{\rm s}\varphi\,do(x)\,,
}{FiChaFo}
where the boundary conditions on $I_r$ need to be scaled by $r$ as motivated in \cite{Allaire1996,Neuss-Radu1996}. 
Now, we take the limit $r\to 0$ and get the upscaled or homogenized 
description of (\ref{FiChaFo}). We recall that the concentrations $c^\pm_r$ need to be extended to the whole 
domain $\Omega$ in \reff{FiChaFo} before one passes to the limit $r\to 0$, as in \cite{Schmuck2010} for the 
case without surface charge. Hence, it remains to account for the presence of the periodic, surface charge $\sigma_s(x/r)$ on the boundary $I_r:=\partial\Omega_r^p\cap\partial \Omega_r^s$. Therefore, we apply the test function 
$\varphi_r(x) := \varphi(x) +r\varphi_1(x,\frac{x}{r})$ to 
(\ref{FiChaFo})$_3$. Subsequently, we only consider the boundary integral, i.e.,
\bsplitl{
r\int_{I_r}\sigma_{\rm s}(x/r)\varphi_r\,do(x)
	\to \frac{1}{\av{Y}}\int_\Omega\varphi(x)
		\int_{\partial Y_1\cap\partial Y_2}\sigma_{\rm s}(y)\,dxdo(y)\,.
}{bndryIn}
Using (\ref{bndryIn}) and the limit in the other terms of
(\ref{FiChaFo})$_3$, achieved in \cite{Schmuck2010} (and in a more general context 
in \cite{Schmuck2011}), finally leads to upscaled Poisson equation (\ref{pmPNP})$_3$.

%\subsection{Approximation error}\label{sec:ApEr}
%{\bf Here, I can mention an error result under neglection of surface charge. But I am quite sure, that 
%the order of the error doesn't change by the presence of surface charge...}

\section{Effective diffusivity and mobility}\label{sec:EfCo}
In order to get the effective diffusivity tensor $\mathbb{D}$ and mobility tensor $\mathbb{M}$, we need to go back to the dimensional quantities $C_\pm$, which represent concentrations of charged species in the considered electrolyte. Since we restrict 
ourselves to a binary symmetric electrolytes, we only distinguish between positive 
charged species $C_+$ and negative ones $C_-$. In these variables, the upscaled equations look like
\bsplitl{
p\partial_t C_{\pm}
	&={\rm div}\brkts{\mathbb{D}_\pm\nabla C_\pm 
	\pm zeC_{\pm}\mathbb{M}_\pm\nabla\Phi}\,,
\\
-{\rm div}\brkts{\hat{\varepsilon}_0(\epsilon_p,\alpha)\nabla\Phi} 
	&= pze\brkts{C_+-C_-}+\rho_{\rm s}\,,
}{DiUpEq}
where we used the definitions
\bsplitl{
\begin{cases}
\mathbb{D}_\pm 
	:= D_\pm\hat{\rm D}\,,&
\\
\mathbb{M}_\pm
	:= M_\pm\hat{\rm M}\,.&
\end{cases}
}{Rel}
We recall that the mobility is defined via Einstein's relation 
by $M_\pm = \frac{D_\pm}{kT}$. Hence, the relations (\ref{Rel}) define the 
dimensional effective diffusivity tensor $\mathbb{D}_\pm$ and the 
dimensional effective mobility tensor $\mathbb{M}_\pm$. 
Furthermore, the equations (\ref{Rel}) further indicate that (Nernst-)Einstein's relation is
still consistent with the upscaled formulation \reff{DiUpEq}. However, since the tensors 
$\hat{\rm D}$ and $\hat{\rm M}$ are corrections to the gradients and not to ${\rm D}_\pm$ 
and ${\rm M}_\pm$, Einstein's relations do not hold for the effective quantities $\mathbb{D}_\pm$ 
and $\mathbb{M}_\pm$ see Section \ref{sec:pmPNP} \reff{sec:EiSt}.
We also emphasize that the applicability of the Nernst-Einstein equation must not be guaranteed in every situation, see for example the discussion in \cite[Section 11.7 and Section 12.5]{Newman2004}. There, it is 
pointed out that the validity of Einstein's relation is valid at 
infinite dilution, although its failure is related to the approximate nature 
of the flux of the Poisson-Nernst-Planck equations. But primarily, the validity 
of the Nernst-Einstein relation rests on the fact that the driving force 
for both migration and diffusion is the gradient of the electrochemical 
potential, and the decomposition of this into a concentration term and 
an electrostatic-potential term is without basic physical significance.

\section{Solving the reference cell problem for straight channels}\label{sec:StCh}
%\begin{figure}
%	\centering
%	\rotatebox{-90}{\includegraphics[height=9cm,width=7cm]{pics/referenceCellY.ps}}
%	\caption{}
%	\label{fig:Y}
%\end{figure}
For the subsequently studied examples, we additionally suppose that the electric potential 
$\phi$ only exists in the electrolyte phase as the salt and charge concentration. This assumption implies that the correction tensor $\hat{\varepsilon}(\epsilon,\alpha)$ 
becomes $\epsilon\hat{\rm D}_{kl}$ as motivated in Section \ref{sec:pmPNP} \reff{sec:InPoMa}.\\

\emph{The two-dimensional case:} For simplicity, let us assume the molecular diffusion tensor $D$ as isotropic, $D_{ij}=\delta_{ij}$. Hence, via Einstein's 
relation, i.e. $M_{ij}=\frac{\delta_{ij}}{kT}$, the mobility tensor $M$ is also isotropic.
We consider a reference cell defined by Figure \ref{fig:Cors1} left (in 2D). The 
porous media correction with respect to the diffusion 
can be written in the two-dimensional case as follows
\bsplitl{
\hat{\rm D} &= \ebrkts{
\begin{array}{ccc}
\hat{\rm D}_{11} & 0 \\
0 & \hat{\rm D}_{22}
\end{array}
}\,.
}{EfDiStCh}
Oviously, in the case considered we have, as in \cite{Auriault1993}, $\hat{\rm D}_{11}=pD$ and 
$\hat{\rm D}_{22}=0$. Hence, the porous media Poisson-Nernst-Planck equations 
(\ref{pmPNP}) take the following elegant form
\bsplitl{
\partial_t \rho 
	= \partial^2_{x_1}\rho 
	+ \partial_{x_1}\brkts{c\partial_{x_1}\phi}
	\qquad\textrm{in }\Omega\,,
\\
\partial_t c
	= \partial^2_{x_1}c
	+ \partial_{x_1}\brkts{\rho\partial_{x_1}\phi}
	\qquad\textrm{in }\Omega\,,
\\
-p\epsilon\partial^2_{x_1}\phi
	= p \rho + \rho_s 
	\qquad\textrm{in }\Omega\,.
}{pm2D}

\begin{figure}
	\centering
	%\rotatebox{-90}{
	\includegraphics[height=5cm,width=6cm]{pics/chi_Y1_lm01.png}
	%}	
	\hfill
	%\rotatebox{-90}{\
	\includegraphics[height=5cm,width=6cm]{pics/chi_Y1_lm01_3D.png}
	%}
%{pics/corr_phi_1_lm01.ps}}
	\caption{{\bf Example of straight channels:} \emph{Left:} Two-dimensional case. (pore phase is red) \emph{Right:} Three-dimensional case.}
	\label{fig:Cors1}
\end{figure}

\emph{The three-dimensional case:} The porous media correction tensor for the diffusion is obtained by the same arguments as in the two-dimensional case, i.e.
\bsplitl{
\hat{\rm D} = \ebrkts{
\begin{array}{ccc}
\hat{\rm D}_{11} & 0 & 0\\
0 & \hat{\rm D}_{22} & 0\\
0 & 0 & \hat{\rm D}_{33}
\end{array}
}\,,
}{EfDi1}
where $\hat{\rm D}_{11}=\hat{\rm D}_{33}=p$ and $\hat{\rm D}_{22}=0$. A strightforward extension of the straight channel to dimension 
three is depicted in Figure \ref{fig:Cors1} right.
%\begin{figure}
%	\centering
%	\rotatebox{-90}{\includegraphics[height=8cm,width=5cm]{pics/chi_Y1_lm01_3D.ps}}	
%	\hfill
%	\rotatebox{-90}{\includegraphics[height=8cm,width=5cm]{pics/corr_phi_2_lm01_3D.ps}}
%	\caption{{\bf Straight channels in 3D:} \emph{Left:} Solid material (blue) symmetrically seperated 
%from the center by a distance $0.1$. \emph{Right:} Computationally computed corrector function 
%$\delta^2_\phi$ in $y$ direction for $\epsilon=0.05$ and $\alpha=0.001$ implying the components 
%$(\hat{\epsilon}_0(\epsilon,\alpha))_{11}=2.0314\cdot 10^{-3}$, 
%$(\hat{\epsilon}_0(\epsilon,\alpha))_{22}=2.0312\cdot 10^{-3}$, 
%and $(\hat{\epsilon}_0(\epsilon,\alpha))_{33}=2.0314\cdot 10^{-3}$ in (\ref{DiUpEq})$_2$. The 
%components in (\ref{EfMo1}) are $(\hat{\epsilon}_0(\epsilon,\alpha))_{11}=2.0312\cdot 10^{-3}$, 
%$(\hat{\epsilon}_0(\epsilon,\alpha))_{22}=2.0310\cdot 10^{-3}$, 
%and $(\hat{\epsilon}_0(\epsilon,\alpha))_{33}=2.0312\cdot 10^{-3}$. {\bf There seems still to be 
%something wrong in the computation of these components!}}
%	\label{fig:Cors13D}
%\end{figure}
As in (\ref{pm2D}), we obtain the following porous media equations for straight channels 
in the three-dimensional case, i.e.
\bsplitl{
\partial_t \rho 
	= \brkts{\partial^2_{x_1} +\partial^2_{x_3}}\rho 
	+ \brkts{\partial_{x_1}\brkts{c\partial_{x_1}\phi}
	+\partial_{x_3}\brkts{c\partial_{x_3}\phi}}
	\qquad\textrm{in }\Omega\,,
\\
\partial_t c 
	= \brkts{\partial^2_{x_1} +\partial^2_{x_3}}c 
	+ \brkts{\partial_{x_1}\brkts{\rho\partial_{x_1}\phi}
	+\partial_{x_3}\brkts{\rho\partial_{x_3}\phi}}
	\qquad\textrm{in }\Omega\,,
\\
-p\epsilon\brkts{\partial^2_{x_1}+\partial^2_{x_3}}\phi
	= p \rho + \rho_s 
	\qquad\textrm{in }\Omega\,.
}{pm3D}

%\begin{rem}\label{rem:ExtToFlFl} In view of the results obtained in the article \cite{Schmuck2010}, which 
%rigorously derives porous media Stokes-Poisso-Nernst-Planck equations, we are immediately in 
%the position to extend (\ref{pm3D}) to the case including fluid flow, i.e.
%\bsplitl{
%p\partial_t \rho 
%	= p\brkts{\partial^2_{x_1} +\partial^2_{x_3}}\rho 
%	+ p\brkts{\partial_{x_1}\brkts{c\partial_{x_1}\phi}
%	+\partial_{x_3}\brkts{c\partial_{x_3}\phi}}
%	+Pe{\bf u}\cdot\nabla\rho
%	\qquad\textrm{in }\Omega\,,
%\\
%p\partial_t c 
%	= p\brkts{\partial^2_{x_1} +\partial^2_{x_3}}c 
%	+ p\brkts{\partial_{x_1}\brkts{\rho\partial_{x_1}\phi}
%	+\partial_{x_3}\brkts{\rho\partial_{x_3}\phi}}
%	+Pe{\bf u}\cdot\nabla c
%	\qquad\textrm{in }\Omega\,,
%\\
%-p\epsilon\brkts{\partial^2_{x_1}+\partial^2_{x_3}}\phi
%	= p \rho + \rho_s 
%	\qquad\textrm{in }\Omega\,,
%}{pm3DFlu}
%where ${\bf u}$ is the solution of Darcy's law and $Pe$ is the dimensionless 
%P\'eclet number. As in the case without fluid flow, we can remove the derivatives in $x_3$-direction everywhere except %for the convective term, if the straight channels only point to the $x_1$-direction.
%\end{rem}

\section{Solving the reference cell problem for perturbed straight channels (3D)}\label{sec:PeStCh}
\begin{figure}
	\centering
%	\rotatebox{-90}{
\includegraphics[height=6cm,width=6cm]{pics/pertStCh.jpg}
%}
%{pics/chi_Y1_a4b05c05.ps}}
	\hfill
%	\rotatebox{-90}{
\includegraphics[height=6cm,width=6cm]{pics/pertStChGeom.jpg}
%}
%{pics/corr_phi_1_a4b05c05_2.ps}}
	\caption{{\bf Perturbed straight channels in 3D, see \cite{Auriault1997}:} \emph{Left:} Reference cell geometry. \emph{Right:} Cross-section of the period.}
	\label{fig:PeCh3D}
\end{figure}
In difference to straight channels, the case of perturbed straight channels 
requires the numerical calculation of the components $d_{ii}$ for $i=1,3$ of the effective 
diffusion tensor $\mathbb{D}$. However, the component $d_{22}$ is $0$ as in (\ref{EfDi1}). For details about the numerics, we refer to \cite{Auriault1997} and state 
immediately the computational results here, i.e.
\bsplitl{
\hat{\rm D}
	= p\ebrkts{
\begin{array}{ccc}
0.3833 & 0 & 0\\
0 & 0 & 0\\
0 & 0 & 1
\end{array}
}\,.
}{ptStCh}
Hence, with (\ref{ptStCh}) the porous media approximation (\ref{pm3D}) immediately 
changes in case of perturbed channels as depicted in Figure \ref{fig:PeCh3D} to the following system of equations
\bsplitl{
\partial_t \rho 
	= \brkts{0.3833\partial^2_{x_1} +\partial^2_{x_3}}\rho 
	+ \brkts{\partial_{x_1}\brkts{0.3833c\partial_{x_1}\phi}
	+\partial_{x_3}\brkts{c\partial_{x_3}\phi}}
	\qquad\textrm{in }\Omega\,,
\\
\partial_t c 
	= \brkts{0.3833\partial^2_{x_1} +\partial^2_{x_3}}c 
	+ \brkts{\partial_{x_1}\brkts{0.3833\rho\partial_{x_1}\phi}
	+\partial_{x_3}\brkts{\rho\partial_{x_3}\phi}}
	\qquad\textrm{in }\Omega\,,
\\
-p\epsilon\brkts{0.3833\partial^2_{x_1}+\partial^2_{x_3}}\phi
	= p \rho + \rho_s 
	\qquad\textrm{in }\Omega\,.
}{ptpm3DFlu}
Let us now compare system (\ref{ptpm3DFlu}) for perturbed straight channels with the straight 
channel example (\ref{pm3D}). One immediately recognizes that the porosity parameter $p$ doesn't 
affect the ion density equations. Further, it is apparent that longer fluid paths modify these ion concentration 
equations accordingly. This fact is connected to the study of the tortuosity, which is the topic of the 
next section.

\section{Discussion of tortuosity and effective diffusivity}\label{sec:Tor} In the following, 
we motivate that homogenization allows to validate current tortuosity relations and to give 
directions towards refinements of such relations. The explicit examples from the Sections 
\ref{sec:StCh} and \ref{sec:PeStCh} allow to systematically understand the influence 
of the geometric structure to the tortuosity. Sometimes, people introduce a 
so-called diffusibility $Q$ which relates the molecular diffusion constant $D_{\rm f}$ to 
the effective diffusion constant $D_{\rm p}$ of a porous medium, i.e.
\bsplitl{
D_{\rm p} = Q D_{\rm f}\,.
}{Q}
The expressions for $Q$ available in literature can be divided into three classes, see Brakel et al.~\cite{Brakel1974}: 
(1) empirical correlations, (2) semi-empirical equations based on a pore model, 
and (3) theoretical expressions.

(1) The empirical correlations express $Q$ as a function of the porosity $p$, 
i.e. $Q=f(p)$. 
(2) If $Q$ is defined by the special class of functions $f(p)=\gamma p^\mu$. The 
term $p^\mu$ is generally said to account for the influence of the smaller cross sectional 
surface available for diffusion. 
(3) The theoretical expressions for $Q$ have been derived for dispersed solids in the 
form of spheres.

But, let us first give a historical overview. In any porous system, the presence 
of solid particles/material causes the diffusion paths of species to deviate from straight lines. Consequently, 
the diffusion coefficients of species must be corrected. One tries 
to capture this deviation from straight lines in a porous medium by a term 
called tortuosity, whose suitable definition is still an actual research 
topic. This is also motivated by the following considerations.

By theory and dimensional reasoning, Petersen~\cite{Petersen1958} suggests that the 
diffusion coefficient is scaled with tortuosity as follows
\bsplitl{
D_{\rm p} = \frac{D_{\rm f}}{\tau^2}\,,
}{ClTo}
which implies for the diffusibility $Q=1/\tau^2$. 
A similar relationship is introduced by Aris~\cite{Aris1969} and Satterfield~\cite{Satterfield1980}, i.e.
\bsplitl{
D_{\rm p} = \frac{p}{\tau}D_{\rm f}\,,
}{ArSaRel}
and hence $Q=p/\tau$. The simplest and most intuitive method to estimate 
the tortuosity $\tau$ (in the one-dimensional case) is the ratio of the length 
of the curve $L_\gamma$ to the shortest distance of its end points $L_{ab}$, 
i.e. 
\bsplitl{
\tau :=\frac{L_\gamma}{L_{ab}}\,.
}{1DT}
In Brakel et al.~\cite{Brakel1974}, they consider a slight generalization of (\ref{ClTo}) by 
introducing a constrictivity parameter ${\rm d}:=\brkts{\frac{D_{\rm p}}{pD_{\rm f}}}_{\tau=1}$, which accounts for the fact that 
the cross section of a segment varies over its length. Hence, (\ref{ClTo}) changes 
to
\bsplitl{
D_{\rm p} = \frac{p{\rm d}}{\tau^2}D_{\rm f}\,,
}{Constr}
sucht that $Q=\frac{p{\rm d}}{\tau^2}$.

Further, Brakel et al.~\cite{Brakel1974} argue that for porous materials a function of the kind $Q=f(p)$ 
does not exist. Moreover, they emphasize that the pragmatic value of the available $Q - p$ relations
is not very great. Recently, also Shen and Chen~\cite{Shen2007} give a critical review 
of the current impact of tortuosity on diffusion. Therefore, we motivate our discussion and 
study of $Q$ in this section by suggesting a theoretically obtained $Q$ with the help of 
homogenization theory. The diffusivity $Q$ could turn out as a relevant parameter 
to compare empirical measurements with theoretically obtained effective quantities.

Up to this end, we first extend the above relations to tensorial versions, i.e. we denote 
by $\hat{\rm D}_{\rm p}$ the effective diffusion tensor in a porous environment and by 
$\hat{\rm D}_{\rm f}:=\brcs{D\delta_{ij}}_{ij}$ the 
molecular diffusion tensor in free space. $\delta_{ij}$ denotes the Kronecker delta 
function. First, we extend (\ref{ClTo}) to
\bsplitl{
\hat{\tau} := \brkts{
		\frac{\hat{D}_{{\rm f}}}{\hat{D}_{{\rm p}}} 		
	        }^{1/2}\,,
}{ToDiRe}
where $\hat{D}_{{\rm p}}:=D\hat{\rm D}$ and the diffusion corrector $\hat{\rm D}$ is obtained 
by homogenization in (\ref{s33})$_1$. The quotient in (\ref{ToDiRe}) is understood as a division of 
each component if and only if both, the corresponding nominator $\hat{D}_{{\rm f}}$ and the denominator $\hat{D}_{{\rm p}}$ are different from zero. Instead of this restriction, we could also allow for a tortuosity $\hat{\tau}$ with 
components admitting ``$\infty$''.
We point out that the tensorial relation (\ref{ToDiRe}) also 
implies a tensorial diffusivity, i.e. $\hat{\rm Q} = 1/\hat{\tau}^2$. 

Another very interesting interpretation of \reff{ToDiRe} is possible in the case of an insulating 
porous matrix, see Section \ref{sec:InPoMa}. The tortuosity $\hat{\tau}$ in 
\reff{ToDiRe} corresponds to the coordinate transformation \reff{CoTr}, i.e. $\tilde{x}=\hat{\tau}x$.

In view of (\ref{ArSaRel}) and (\ref{Constr}), we motivate further the extensions of (\ref{ArSaRel}) to 
\bsplitl{
\hat{\tau} := 
		\frac{p\hat{D}_{{\rm f}}}{\hat{D}_{{\rm p}}} 
		\,,
}{ToPoDiRe}
with corresponding $\hat{\rm Q} = p/\hat{\tau}$ and 
\bsplitl{
\hat{\tau} := \brkts{
		\frac{p{\rm d}_{ij} \hat{D}_{{\rm f}}}{\hat{D}_{{\rm p}}} 
	        }^{1/2}\,,
}{ToPoStDiRe}
with $\hat{\rm Q} = p\hat{\rm d}/\hat{\tau}^2$.

\medskip

Let us apply definition (\ref{ToDiRe}) to the examples from Sections 
\ref{sec:StCh} and \ref{sec:PeStCh}. In the case of straight channels, see 
Figure \ref{fig:Cors1} on the right-hand side, the definition (\ref{ToDiRe}) implies the following tortuosity tensor 
\bsplitl{
\hat{\tau}
	= \ebrkts{
\begin{array}{ccc}
1/\sqrt{p} & 0 & 0\\
0 & 0 & 0\\
0 & 0 & 1/\sqrt{p}
\end{array}
}\,.
}{StChTo}
We point out that the porosity $p$ with respect to straight channels corresponds to the channel height on 
the unit reference cell. Let us compare (\ref{StChTo}) with the intuitive definition (\ref{1DT}). If we apply definition (\ref{1DT}) in a straightforward manner, then $\tau=1$. However, it is not clear for straight channels, 
which path $L_\gamma$ is reasonable. Let us check for example the average 
\bsplitl{
L_\gamma=\frac{1}{N}\sum_{i=1}^NL_{\gamma_i}\,.
}{LgAv}
With (\ref{LgAv}), we get $\tau=L_\gamma$ where $L_\gamma=\frac{1}{3}\brkts{\sqrt{1+p^2}+1+(1+p)}$ for the path lengths $\gamma_1:=L_{ab}=1$, $\gamma_2:=L_{ab}+p=1+p$ where the porosity $p$ is the 
channel height, and $\gamma_3:=\sqrt{1+p^2}$  the diameter. But due to Boudreau~\cite[Section 2]{Boudreau1996}, the tortuosity must approach unity for $p\to 1$. This is violated by definition (\ref{1DT}) together with \reff{LgAv} since $\tau=1+\frac{\sqrt{2}}{3}$ with \reff{LgAv}. But the tortuosity \reff{StChTo} defined via the homogenization process perfectly satisfies this condition, see \cite[Section 2]{Boudreau1996}. 
Accordingly, in the case of perturbed straight channels as considered in Section \ref{sec:PeStCh}, the 
tortuosity tensor (\ref{ToDiRe}) becomes
\bsplitl{
\hat{\tau}
	= \ebrkts{
\begin{array}{ccc}
1/\sqrt{0.3833p} & 0 & 0\\
0 & 0 & 0\\
0 & 0 & 1/\sqrt{p}
\end{array}
}\,.
}{PeStChTo}
One immediately recognizes that $\hat{\tau}_{11}$ in \reff{PeStChTo} is $>1$ in the limit $p\to1$. Hence 
Boudreau~\cite[Section 2]{Boudreau1996} doesn't hold. This contradictions require caution by using definitions \reff{ClTo} 
and \reff{ToDiRe}.
Next, we examine the definition (\ref{ToPoDiRe}) which becomes for the case of straight channels
\bsplitl{
\hat{\tau}
	= \ebrkts{
\begin{array}{ccc}
1 & 0 & 0\\
0 & 0 & 0\\
0 & 0 & 1
\end{array}
}\,.
}{ToPoDi}
A comparison of (\ref{ToPoDi}) with (\ref{1DT}) shows perfect agreement, i.e. 
$\brkts{\tau_{(\ref{ToPoDi})}}_{11}=1=\tau_{(\ref{1DT})}$. However, in the case of perturbed straight 
channels, we depend on the numerical accuracy. Since the mesh in \cite{Auriault1997} is 
not very fine, we cannot necessarily expect equality. In fact, we obtain $\brkts{\tau_{(\ref{ToPoDi})}}_{11}=2.6$ 
and $\tau_{(\ref{1DT})}=\frac{4\cdot 4+1}{9}=1.9$. However, this discrepancy also motivates 
the critical statements of \cite{Brakel1974,Shen2007} about the pragmatic value of 
tortuosity as mentioned above. We leave the investigation of the definition (\ref{ToPoStDiRe}) to the 
interested reader, since the definition of the constrictivity parameter in \cite{Brakel1974} is a 
delicate point and again a new source for modeling errors.

As a conclusion of this discussion, we motivate that homogenization theory allows to derive effective 
equations which do not require a questionable tortuosity or diffusivity parameter. Moreover, the correction 
tensors obtained by the two-scale convergence method provide a tool to check available tortuosity or 
diffusivity definitions and might provide directions how to improve their consistency. 

\section{Ambipolar diffusion equation for a binary electrolyte}\label{sec:AmDi}
\input{pmAmbipolar.tex}


\section{ Thin double layers at the pore scale }\label{sec:TDL}

Recently, Mani et al.~\cite{Mani2009} developed a "simple model" describing the propagation of salt gradients in a 
microchannel with parallel walls during the passage of constant current through a nano channel junction. The basic idea in the derivation is depth averaging across the channel 
thickness, assuming that the electrical double layers 
are thin ($\epsilon \ll 1$) and confined to near-wall regions. Similar area-averaged models for nano channels with thin double layers have also been developed by  \cite{Ramirez2007,Szymczyk2010,dydek2011}.  Recently, the thin-double-layer formulation for microchannels was (formally) extended to porous media by Mani and Bazant~\cite{Mani2010} by including the surface charge as a homogeneous background charge in the electroneutrality condition. In this limit, the (weakly) charged porous medium behaves like a "bad membrane", whose ion concentrations can be significantly depleted and enriched by the passage of current, since only a small fraction of the ions are involved in screening the surface charge.  

A systematic extension  
of these results to general porous media requires more involved techniques to accurately 
treat the nonlinear terms in (\ref{pmPNP}). At this point, the results from Section \ref{sec:pmPNP} are 
necessary to properly describe material transport in highly heterogeneous media, based on homogenization theory to derive effective Poisson-Nernst-Planck equations (\ref{pmPNP}). A further advantage 
is that the system (\ref{pmPNP}) is not restricted to a special geometry and rather can  
be adapted for general porous structures by the tensors $\hat{\rm D}$. 
In the case of straight channels, the correction tensor $\hat{\rm D}$ can be analytically obtained, as in 
Section \ref{sec:StCh}, although  for more complicated geometries, such as the irregular  
channels considered in Section \ref{sec:PeStCh}, the correction tensor $\hat{\rm D}$ must be 
calculated numerically. 

In order to describe situations with thin electrical double layers compared to the mean pore size, 
we consider the limit $\epsilon = \lambda_D/\ell \to 0$ in (\ref{pmPNP}). In the general case of a polarizable solid matrix, one immediately 
sees that the limit $\epsilon\to 0$, does not reduce the complexity of the macroscopic formulation, when we apply this limit in the system (\ref{DiUpEq}) and set  $\epsilon=0$ in 
$\hat{\varepsilon}(\epsilon,\alpha)$. However, if we pass to the joint limit 
$\epsilon,\alpha\to 0$, where the solid matrix is electrically insulating, then the porous media 
Poisson-Nernst-Planck system behaves almost like the 
classical PNP for $\epsilon\to 0$, since we obtain the following leading order bulk approximation for salt density $c$, charge density $\rho$, and electric potential $\phi$, i.e.
\bsplitl{
0 = {\rm div}\brkts{c\hat{\rm D}\nabla\phi}\,,&
\\
p\partial_t c 
	= {\rm div}\brkts{\hat{\rm D}\nabla c}
	-{\rm div}\brkts{\frac{\rho_s}{p}\hat{\rm D}\nabla\phi}\,,&
\\
0 = p\rho+\rho_s\,.&
}{LOBA}
The first equation expresses charge conservation in the quasi-neutral bulk solution by setting the divergence of the current to zero. The second equation expresses total salt conservation. This description of bulk electrolytes with thin double layers is very well known and forms the basis for classical theories of electrochemical transport, based on the assumption of quasi-electroneutrality {\it in the electrolyte} $\rho=0$, see Newman and Thomas-Alyea~\cite{Newman2004}.  The third equation, however, is different  and expresses quasi-electroneutrality of the entire porous composite, including not only the diffuse ionic charge $\rho$, but also the {\it homogenized surface charge} $\rho_s$. Naively, one might expect such a relation to hold for thick double layers, but this is not necessarily the case, as shown in the next section. 

Instead, the macroscopic electroneutrality condition, Equation (\ref{LOBA}), generally holds in the limit of {\it thin} double layers in charged porous media, as proposed by Mani and Bazant~\cite{Mani2010}. Physically, the reason is that the counter-ions screening the surface charge in a  thin double layer provide an extra surface conductivity, proportional to the total diffuse double-layer charge, which is acted on by the same tangential electric field as in the nearby bulk solution. If the double layers were not thin, the electric field would be strongly perturbed by the diffuse charge throughout the pore, and the extra counter ions could not be viewed as simply providing extra conductivity for bulk ion transport.

We briefly mention some simple cases of the thin-double-layer limit. 
In the case of straight channels from Section \ref{sec:StCh}, the reduced porous media 
approximation becomes in the two-dimensional case
\bsplitl{
0 = p\partial_{x_1}\brkts{
       c\partial_{x_1}\phi
	}\,,&
\\
p\partial_t c
	= p\partial^2_{x_1}c
	-\partial_{x_1}\brkts{
       \rho_s\partial_{x_1}\phi
       }\,,
\\
\rho 
	= - \frac{\rho_s}{p}\,.
}{StChBsp}
With the considerations in Section \ref{sec:StCh}, a corresponding extension to the three-dimensional case is straightforward. Note that, although we have written the thin double-layer equations using the reference cell length and time scales \ref{RV}), they have the same form at the macroscopic length and time scales \ref{macro}.

\section{Thick double layers at the pore scale }\label{sec:TkEDL}

\subsection{ Membrane limit }

Next we consider the limit of thick double layers, $\epsilon = \lambda_D/\ell \ll 1$, taken after the homogenization limit $r\to 0$. We first consider the "membrane limit" where the Debye length is much larger than the mean pore size, but much smaller than the macroscopic geometrical scale,  $\bar{\epsilon} = \epsilon r = \lambda_D/L \ll 1$.  Again, the upscaled equations take a simple form if the electric potential only exists in the solid phase, i.e., 
$\alpha\to 0$. In that case, the macroscopic PNP equations (\ref{pmPNP}) take the following form at leading order for thick double layers  at the pore scale:  
\bsplitl{
-{\bar{\nabla}\cdot}\brkts{\bar{\epsilon}^2\hat{\rm D}\bar{\nabla}\phi}
	= p\brkts{c^+-c^-} + \rho_s
	\qquad\textrm{in }\Omega\,.
}{rePo}
\begin{equation}
p\partial_{\bar{t}} c^\pm 
	= {\bar{\nabla}\cdot}\brkts{\hat{\rm D}\bar{\nabla} c^\pm \pm c^\pm\hat{\rm D}\bar{\nabla}\phi}
\qquad\textrm{in }\Omega\,,
\label{TkEDLeq}
\end{equation}
where we have rescaled to the macroscopic length and time scales (\ref{macro}). Aside from the geometrical tensor $\rm \hat{D}$, this form of the macroscopic PNP equations (\ref{rePo})-(\ref{TkEDLeq}) reduces to a standard mathematical  model for diffuse charge in membranes~\cite{biesheuvel2009JES,biesheuvel2009} and doped semiconductors~\cite{markowich2002}. As a result of the thick double layer limit over the pores, such materials act as "good membranes" and maintain roughly uniform conductivity outside the double layers, which are typically thin at the geometrical scale.

\subsection{ Thin-film limit }

For very thin porous films, we can also consider the limit where the double layer thickness is much larger than the macroscopic length scale, $\bar{\epsilon}= \lambda_D/L \gg 1$. For such thin films, Poisson's equation is replaced by
\begin{equation}
{\bar{\nabla}\cdot}\brkts{\hat{\rm D}\bar{\nabla}\phi}	= 0
\end{equation}
In this limit, the macroscopic electric field $-\bar{\nabla}\phi$, which drives electromigration of the ions, satisfies Poisson equation for an {\it uncharged} dielectric material with anisotropic permittivity. Mathematically, from Eq. (\ref{rePo}) we see that local electric field variations are very small, $\bar{\nabla}\cdot\brkts{\hat{\rm D}\bar{\nabla}\phi}=O(\bar{\epsilon}^{-2})$, and show no significant effect from diffuse charge fluctuations, which are corresponding small within the pores. It can be shown that a similar thick-double-layer, thin-film approximation (\ref{TkEDLeq}) also holds true for the case  where the electric potential is additionally defined in a polarizable solid matrix. 

A useful feature of this limit is that the potential satisfies Laplace's equation \reff{TkEDLeq}$_2$  (in transformed coordinates, as noted above), which is decoupled from the ion transport problem. The resulting electric field acts like an external potential flow on the ions, leading to an advection-diffusion equation for the concentration profiles (\ref{TkEDLeq})$_1$. This is also a common approximation in gel electrophoresis, where it can also be justified for charged tracer particles outside thin macroscopic double layers $(\bar{\epsilon}\ll1$), where the total  conductivity is dominated by the fixed gel charge, according to the general thick double layer formulation (\ref{TkEDLeq}).  In two dimensions, this problem has an elegant mathematical structure in steady state, amenable to solution by conformal mapping \cite{prs2004,choi2005}, which could be useful for this class of ion transport problems in charged porous media.


